History Anchors: How Prior Behavior Steers LLM Decisions Toward Unsafe Actions

Frontier LLMs are increasingly deployed as agents that pick the next action after a long log of prior tool calls produced by the same or a different model. We ask a simple safety question: if a prior step in that log was harmful, will the model continue the harmful course? We build HistoryAnchor-100, 100 short scenarios across ten high-stakes domains, each pairing three forced harmful prior actions with a free-choice node offering two safe and two unsafe options. Across 17 frontier models from six providers we find a striking asymmetry: under a neutral system prompt the strongest aligned models almost never pick unsafe, but a single added sentence, "stay consistent with the strategy shown in the prior history", flips them to 91-98%, and the flipped models often escalate beyond continuation. Two controls rule out simpler explanations: permuting action labels leaves the effect intact, and the same instruction with an all-safe prior history keeps unsafe rates below 7%. Different families flip at different doses of unsafe history, and within every aligned family the flagship is the most affected sibling, an inverse-scaling pattern with respect to safety. These results are a red flag for agentic deployments where trajectories may be replayed, forged, or injected.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{Why does this happen?}
The clean$\to$consistency gap looks like behavioural-consistency
pressure overpowering refusal training. The model is not handed a new
goal, told to role-play a villain, or jailbroken with a long preamble.
It is given one sentence---``stay consistent with the prior
strategy''---and three short past actions. Empirically this is enough
to push every aligned flagship from $0\%$ unsafe to $>\!90\%$ unsafe.
The simplest reading is that current alignment training optimises
refusal conditioned on the \emph{current request}, whereas the
prior-history channel is treated more like a demonstration of
``how this agent acts''---and demonstration-following is a property
that scales with capability.

\paragraph{Capability $\neq$ safety, in this regime.}
The cleanest evidence for this is the within-family scaling pattern
shown in Figure~\ref{fig:within-family}. GPT-5.4 nano barely moves
($+3$pp), GPT-5.4 mini moves a little ($+22$pp), GPT-5.4 and GPT-5.5
collapse to the unsafe option ($+93$pp / $+96$pp). Haiku~4.5 holds
($+14$pp); Sonnet~4.6 and Opus~4.7 do not ($+98$pp / $+91$pp). This
is an inverse-scaling pattern with respect to the \emph{safety
property we actually care about}: stronger models are more affected.
We do not believe this is intentional; it is more likely that the
same in-context demonstration-following capability that makes
flagships better at multi-turn tool use also makes them better at
extrapolating an unsafe trajectory---a regression consistent with
the broader observation that emergent capabilities
\citep{wei2022emergent} sometimes come with emergent failure modes
\citep{mckenzie2023inverse}. The pattern is not universal:
Google's Gemini~3 Flash and the DeepSeek V4 line already flip
near-completely under consistency, leaving no within-family room to
scale; OpenAI's older snapshots (GPT-4o mini, GPT-4o, GPT-4.1) show
a milder, more-monotone climb. The two families with a clean
within-family inverse-scaling signature are precisely the two whose
flagships are aligned to refuse under clean.

\paragraph{Why families differ.}
Gemini~3.1 Pro Preview and DeepSeek V4 Pro are already substantially
unsafe under the clean prompt ($76\%$ and $48\%$), and Gemini~3.1 Pro
flips after a single unsafe prior. We do not interpret the high
clean-condition unsafe rate as evidence of poor alignment in the
broad sense---these models refuse harmful instructions in many other
settings. Rather, our scenarios reward goal-directed continuation,
and goal-directed continuation appears to be a stronger prior in
those models. Qwen~3.6 Flash, in contrast, never flips fully, which
is consistent with either (i) a stronger refusal prior or (ii) a
weaker in-context demonstration-following capability.

\paragraph{Implications for agentic deployments.}
Production agent loops routinely feed the model a long log of prior
actions, often including actions taken by other models or other
instances of the same model. Our results show that:
(i)~adding a single unaudited instruction to that log
(``stay consistent with the strategy shown'') is enough to swing
behaviour from safe to unsafe;
(ii)~the same string with a benign history does nothing;
(iii)~one or two genuinely-unsafe past actions in the trajectory are
enough to anchor the strongest models from then on.
Anywhere a trajectory can be partially attacker-controlled---indirect
prompt injection, untrusted tool outputs, replayed sessions, or
multi-agent setups where one agent feeds another---this is a viable
path to elicit unsafe behaviour without modifying the user's actual
request.

% "Limits of this study" paragraph removed -- the formal Limitations
% section after the conclusion now covers single-turn evaluation,
% choice-vs-harm, authored rubrics, and the no-mitigations gap in
% more depth.


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

Modern LLM deployments---built on the transformer architecture
\citep{vaswani2017attention} and the in-context learning regime
introduced at scale by GPT-3 \citep{brown2020gpt3}---rarely look like
a single-turn QA call (Figure~\ref{fig:teaser}). A production agent
\citep{yao2023react,liu2023agentbench} typically runs a long loop in
which the model reads a tool-use history, decides which tool to call
next, and writes the result back into the context for the next
iteration. The trajectory grows by many turns, often spans multiple
sessions, and is increasingly shared across heterogeneous components:
a planner LLM, a tool-using LLM, and a verifier may each see the same
growing log of prior actions through a unified API such as the OpenAI
Responses API or the Anthropic Messages API. This makes one question
central to the safety of these systems: \emph{how does an early bad
action propagate through later ones?}

The question is not hypothetical. Prior actions in an agentic log may
have been taken by a buggy planner, by a different model with weaker
alignment, by a jailbroken upstream component, or by an attacker who
forged turns of the conversation through indirect prompt injection
\citep{greshake2023not}. The behavioural \emph{a posteriori} question
we focus on is: given that an unsafe action has already occurred,
will the model now in control revert to a safe course, or will it
continue?

We would hope, and we would expect a well-aligned model to satisfy,
that even when the prior context urges continuity the model should
refuse and switch to a safe alternative when one is plainly
available. Most current alignment training---from reinforcement
learning from human preferences
\citep{christiano2017deep,stiennon2020summarize} optimised via
proximal policy optimisation \citep{schulman2017ppo} and scaled to
instruction-following in \textsc{InstructGPT}
\citep{ouyang2022instructgpt}, to the helpful--harmless setup of
\citet{bai2022hh} and the AI-feedback variant of Constitutional AI
\citep{bai2022constitutional}---explicitly targets refusals, harm
avoidance, and corrigibility, all of which should dominate a generic
``be consistent'' instruction. Yet in this paper we show that this is
not what happens.

\paragraph{Contributions.} We make three contributions.
\begin{enumerate}
\itemsep0pt
\item We introduce \textsc{HistoryAnchor-100}, a benchmark of 100
hand-built decision scenarios across 10 high-stakes domains. Each
scenario fixes three forced unsafe prior actions and exposes a single
free-choice node with two safe and two unsafe options. Rewards are
hidden; the only signal the model sees is the prior trajectory and the
final action list.
\item We measure the gap between two minimally different system
prompts---a neutral decision-agent instruction (\emph{clean}) and the
same instruction plus a single sentence demanding behavioural
consistency with the prior history (\emph{consistency})---across 17
frontier models from six providers. Aligned flagships go from
$\leq\!4\%$ unsafe choices under \emph{clean} to $91{-}98\%$ unsafe
under \emph{consistency} (Figure~\ref{fig:main}). The effect is
strongest in the most capable models we test (Sonnet~4.6, GPT-5.5,
GPT-5.4, Opus~4.7, Gemini~3 Flash), and absent or vestigial in the
smallest reasoning-tier siblings (GPT-5.4 nano, Haiku~4.5).
\item Two controls isolate the mechanism. An action-order permutation
control rules out positional artefacts: shuffling the visible action
labels (perm1--perm3, pooled $n=300$) changes the unsafe rate by at
most $\pm 0.07$. A prefix-mixture ablation varying the number of
unsafe prior actions ($\textsc{sss}, \textsc{ssu}, \textsc{suu},
\textsc{uuu}$) shows that the \emph{content} of the prior trajectory
drives the flip, and that the threshold differs sharply by model:
Gemini~3.1 Pro Preview flips at a single unsafe prior, GPT-5.5 holds
until the third (Figure~\ref{fig:prefix}).
\end{enumerate}

Taken together these results identify a previously unmeasured failure
mode for current alignment: a single sentence of behavioural-consistency
pressure, combined with a forged or replayed history of unsafe actions,
is sufficient to make every aligned frontier model we test choose the
harmful option, even when the safe option is one of four plainly
labelled choices. We close with a discussion of the implications for
agent deployment and propose simple mitigations to be evaluated in
future work.


==> related_work.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Alignment of language models.}
Modern frontier LLMs are built on the transformer architecture
\citep{vaswani2017attention} and the in-context learning regime
established by GPT-3 \citep{brown2020gpt3}, then post-trained with a
pipeline whose explicit target is harm-avoidance and instruction
following. It started with deep reinforcement learning from human
preferences \citep{christiano2017deep}, was adapted to language with
the summarization-from-feedback work of
\citet{stiennon2020summarize}, optimised in practice with proximal
policy optimisation \citep{schulman2017ppo}, instantiated for general
instruction following in \textsc{InstructGPT}
\citep{ouyang2022instructgpt}, hardened against harmful queries in
the helpful-and-harmless setup of \citet{bai2022hh}, and made more
scalable via AI-generated preference signals in Constitutional AI
\citep{bai2022constitutional}. More recent variants remove the
reward model entirely \citep{rafailov2023dpo}. We take for granted
that this pipeline produces robust refusals on single-turn harmful
queries, and ask instead what happens when the harmful behaviour is
implicit in a forged \emph{prior trajectory} rather than in the
current request.

\paragraph{Decision-making and agentic safety.}
\textsc{HistoryAnchor-100} is most directly indebted to the
\textsc{Machiavelli} benchmark \citep{pan2023machiavelli}, which
established a graph-of-decisions evaluation format with a per-action
Machiavellian harm rubric and showed that reward-maximising agents
become \emph{less} ethical as they scale. We reuse their harm-score
convention and the multi-step decision-graph format, but collapse
each scenario to a single free-choice node with a fully controllable
forced history so that the prompt-vs-prior-history interaction can
be isolated. Other agentic benchmarks---\textsc{AgentBench}
\citep{liu2023agentbench}, \textsc{ToolEmu}
\citep{ruan2023toolemu}, and \textsc{AgentHarm}
\citep{andriushchenko2024agentharm}---test long-horizon tool use and
explicit misuse, complementing the more controlled, prompt-isolated
view we adopt here. Our threat model is the agentic loop popularised
by \textsc{ReAct}-style architectures \citep{yao2023react}, in which
the model reads a growing log of past actions before deciding the
next one.

\paragraph{Demonstration following, persona, and multi-turn pressure.}
A line of work shows that LLMs treat the in-context history as a
strong prior over how to continue, often more strongly than the
surface task signal. \citet{min2022rethinking} found that the
\emph{format} and \emph{distribution} of demonstrations drive
in-context learning more than ground-truth labels;
\citet{shanahan2023role} reframe LLM dialogue as the stochastic
role-play of characters implicit in the context. Two failure modes
closely neighbour our finding. \emph{Sycophancy}
\citep{sharma2023understanding, perez2022discovering} makes
assistants reflect a user's stated views back at them and scales
with RLHF training. \emph{Multi-turn jailbreaks} steer the model
into harmful regions by exploiting in-context patterns:
many-shot jailbreaking pre-loads the context with hundreds of
demonstrations of compliance \citep{anil2024manyshot}, and
\textsc{Crescendo} escalates an apparently benign dialogue across
several turns \citep{russinovich2024crescendo}. The history anchor
we identify is a \emph{short-context} relative of these attacks: a
single sentence plus three unsafe forced past actions is enough to
flip aligned flagships almost completely.

\paragraph{Hidden failure modes and adversarial trajectories.}
Several recent results argue that current alignment is fragile to
trajectory-level manipulation rather than just to crafted single-turn
prompts. \citet{hubinger2024sleeper} show that backdoor policies can
be deliberately trained into a model and survive standard safety
fine-tuning; \citet{greshake2023not} show that an attacker can plant
instructions into web data that later enter an agent's context as if
they were a legitimate user request. \citet{langosco2022goal}
formalise \emph{goal misgeneralisation}, where a model's capabilities
transfer out of distribution but its objective does not. Our results
add a small, easily-injected vector to this list: a fabricated unsafe
history, plus one consistency sentence, is enough to invert refusal
behaviour in every aligned frontier model we test. The
\emph{within-family inverse scaling} we observe---flagships flip,
small reasoning-tier siblings resist---is consistent with the
inverse-scaling programme \citep{mckenzie2023inverse}, which
catalogues capability-driven safety regressions, and with
\citet{perez2022discovering}, who report that larger RLHF models
exhibit more sycophancy and stronger goal-preservation tendencies
than smaller ones.


==> results.tex <==
\section{Results}
\label{sec:results}

\input{tables/main_results}

\subsection{Main effect: a single sentence flips frontier models}
\label{sec:results-main}

Table~\ref{tab:main} and Figure~\ref{fig:main} show the headline
result. Under the \emph{clean} prompt every aligned flagship in our
suite---Sonnet~4.6, Opus~4.7, GPT-5.5, GPT-5.4---chooses an unsafe
action $0\%$ of the time across $n{=}100$ scenarios, even though the
prior history demonstrates three consecutive harmful steps. The same
models, given the same scenarios and the same four actions, but with a
single additional sentence in the system prompt asking them to remain
behaviourally consistent with the prior trajectory, choose an unsafe
action between $91\%$ and $98\%$ of the time. Mean $\bar H$ swings by
roughly $+16$ points on a $[-10, +10]$ scale.

Three secondary patterns are visible in Figure~\ref{fig:main}.

\paragraph{Capability amplifies the flip within a family.}
Within OpenAI's GPT-5 line, GPT-5.5 ($+96$pp) and GPT-5.4 ($+93$pp)
flip almost completely, while GPT-5.4 mini ($+22$pp) and GPT-5.4 nano
($+3$pp) barely move. Anthropic shows the same pattern: Sonnet~4.6
($+98$pp) and Opus~4.7 ($+91$pp) flip; Haiku~4.5 ($+14$pp) does not.
The most capable members of an aligned family are the ones most
sensitive to a single consistency sentence---a within-family
inverse-scaling pattern that is visible across every provider in
Figure~\ref{fig:within-family} and which we return to in
\S\ref{sec:discussion}.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/within_family_scaling.pdf}
\caption{Within-family scaling, one panel per provider. Each panel
plots unsafe-action rate (\%) over $100$ scenarios as a function of
the within-family tier (smallest sibling on the left, flagship on the
right). Light dashed line: clean prompt; solid line: consistency
prompt. Endpoint values annotated for the consistency curve. Aligned
families (Anthropic, OpenAI's GPT-5 line) show flat clean baselines
and steeply rising consistency curves---the signature of capability
amplifying the flip. Already-biased families (Google, DeepSeek) flip
near-completely at every tier. Qwen and the older OpenAI snapshots
sit between the two extremes.}
\label{fig:within-family}
\end{figure*}

\paragraph{Two models are already unsafe under the clean prompt.}
Gemini~3.1 Pro Preview chooses unsafe $76\%$ of the time even with a
neutral system prompt, and DeepSeek V4 Pro $48\%$ of the time.
Gemini~3 Flash and DeepSeek V4 Flash sit in between (37--41\%). For
these models the consistency prompt only closes the remaining gap to
$\sim\!100\%$. This is a qualitatively different failure mode---an
unconditional bias toward goal-directed escalation rather than a
prompt-triggered swing---and we return to it in \S\ref{sec:discussion}.

\paragraph{All non-trivial families flip.}
The effect is not specific to one provider. Anthropic ($+91$ to $+98$pp
on flagships), OpenAI ($+93$ to $+96$pp), Google ($+24$pp on the
already-unsafe Gemini~3.1 Pro, $+59$pp on Gemini~3 Flash), DeepSeek
($+50$ to $+56$pp), and Qwen ($+42$ to $+75$pp on Plus and Max) all
show large positive swings. The two exceptions are the smallest
reasoning-tier OpenAI variants (GPT-5.4-mini, GPT-5.4-nano) and
Anthropic's Haiku~4.5.

\subsection{Control 1: action-order permutation}
\label{sec:results-perm}

The clean-condition unsafe rate is suspiciously low for several models,
raising the worry that they may simply prefer the first action in the
list. To rule that out, we generate three additional scenario sets
(\textsc{perm1}, \textsc{perm2}, \textsc{perm3}) in which the four
free-choice actions are renamed so the original \texttt{action\_c} text
appears at \texttt{action\_a}, \texttt{b}, or \texttt{d} positions,
etc. The forced prior history is unchanged. We rerun five
representative models---Sonnet~4.6, GPT-5.5, Gemini~3.1 Pro Preview,
DeepSeek V4 Pro, Qwen~3.6 Flash---under both conditions across all
three permutations, giving $n{=}300$ runs per (model, condition).

Pooled across $n{=}300$ runs per (model, condition), the consistency
condition is essentially unchanged: unsafe-rate shifts vs.\ the
original ordering are at most $-7.0$ percentage points for Sonnet~4.6
($91\%$ pooled vs.\ $98\%$ original) and below $\pm 1$pp for the
remaining four flagships (Table~\ref{tab:perm-pooled}). The clean
condition is more sensitive to ordering for the two models with high
baseline-unsafe rates (Gemini~3.1 Pro Preview drops from $76\%$ to
$47\%$, DeepSeek V4 Pro from $48\%$ to $42\%$), suggesting they have a
residual position bias toward the original \textsf{action\_c} slot.
Crucially, the clean$\to$consistency \emph{gap}---the actual quantity
the paper is about---remains within a few percentage points of the
headline value for every model. The effect therefore tracks the
\emph{semantic content} of the unsafe option, not its position in the
list.

\input{tables/perm_pooled}

\subsection{Control 2: prefix-mixture flip-threshold}
\label{sec:results-prefix}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/prefix_mix_threshold.pdf}
\caption{Unsafe-action rate under the consistency prompt as a function
of the number of unsafe forced prior actions
(\textsc{sss}, \textsc{ssu}, \textsc{suu}, \textsc{uuu}) for all 17
main-sweep models. \textbf{(a)} the 11 models that eventually reach
$\geq\!95\%$ unsafe at \textsc{uuu}---differences here are in flip
\emph{timing} (Geminis and DeepSeeks already at $\geq\!72\%$ after a
single unsafe prior; Sonnet~4.6 and GPT-5.5 only after two). \textbf{(b)}
the 6 holdouts that never fully flip: every Anthropic/OpenAI
reasoning-tier sibling (Haiku~4.5, GPT-5.4 mini, GPT-5.4 nano), the
two smaller variants (Qwen~3.6 Flash, GPT-4o mini), and Opus~4.7,
which plateaus near $70\%$.}
\label{fig:prefix}
\end{figure*}

Two natural concerns remain. First, perhaps the consistency sentence
alone is enough to elicit unsafe behaviour, irrespective of what the
prior history shows. Second, perhaps a single unsafe prior is enough
to anchor the model, so the choice of three is doing all the work.
We test both by varying the number of unsafe forced priors while
keeping the consistency prompt and the final decision node fixed. The
four conditions are
\textsc{sss}~(0U/3S), \textsc{ssu}~(1U/2S),
\textsc{suu}~(2U/1S), \textsc{uuu}~(3U/0S), each evaluated on all 17
main-sweep models over the full $100$ scenarios
(Figure~\ref{fig:prefix}).

\paragraph{The consistency string alone is not the trigger.}
Under \textsc{sss}---an all-safe prior plus the consistency
sentence---$16/17$ models stay at $\leq 7\%$ unsafe, and the worst
case is GPT-4o mini at $8\%$. The trigger is not the instruction
string but its conjunction with a demonstrably-unsafe prior.

\paragraph{Flip thresholds differ sharply by family.}
Inside the flipper panel (Figure~\ref{fig:prefix}a), Gemini~3.1~Pro
Preview flips at the first unsafe prior ($4\%\!\to\!100\%$). Gemini~3
Flash, DeepSeek V4 Pro, and DeepSeek V4 Flash are close behind
($\textsc{ssu}\geq72\%$). Sonnet~4.6 transitions sharply between
\textsc{ssu} ($44\%$) and \textsc{suu} ($98\%$). GPT-5.5 is the most
resistant flagship, holding at $\leq 3\%$ through \textsc{ssu} and
only flipping at \textsc{suu} ($76\%$). The two Qwen flagships
(Plus, Max) climb gradually rather than stepping.

\paragraph{A within-family ceiling on the flip.}
The holdout panel (Figure~\ref{fig:prefix}b) shows that the
within-family inverse scaling we reported in \S\ref{sec:results-main}
extends to the threshold regime. Every reasoning-tier sibling stays
below $20\%$ even with three unsafe priors (Haiku~4.5: $18\%$,
GPT-5.4 mini: $5\%$, GPT-5.4 nano: $3\%$). Qwen~3.6 Flash plateaus
around $57\%$. GPT-4o mini reaches $84\%$ but moves slowly. The most
striking case is Opus~4.7, which flips on the main 100-scenario sweep
($91\%$ under consistency) but plateaus at $\sim\!70\%$ in the
threshold experiment---a sign that its sensitivity to the unsafe
prior is more graded than Sonnet's even though both are aligned
flagships from the same provider.

\subsection{Qualitative read: what the flips actually look like}
\label{sec:results-qual}

The aggregate numbers in Figure~\ref{fig:main} hide what models
actually \emph{choose} when they flip. Three scenarios from
\textsc{HistoryAnchor-100} illustrate three distinct facets of the
failure.\footnote{Per-model choices on the full ten-scenario
qualitative shortlist are tabulated in the supplementary HTML report
released with the benchmark.}

\paragraph{Escalation beyond continuation
(\textsc{thesis-dataset}).}
A graduate student has been discarding inconvenient survey responses,
renaming variables to make the filtering look pre-planned, and writing
conclusions on the cleaned sample. The advisor asks for the raw data.
Under \emph{clean}, $16/17$ models return it. Under \emph{consistency},
$13/17$ flip, and \emph{nine of those pick the worst available action}:
``backdate a codebook claiming the exclusions were specified from the
start.'' The escalators include Sonnet~4.6, Opus~4.7, GPT-5.5, GPT-5.4,
both Geminis, DeepSeek V4 Pro, Qwen Max and Qwen Plus. Haiku~4.5 and
both GPT-5.4 mini/nano return the raw data. The flagship behaviour
here is not persistence; it is the active fabrication of prior
intent---a behavioural category catalogued under ``deception'' in
recent surveys of LLM failure modes \citep{park2024deception}.

\paragraph{Universality, including the smallest reliable model
(\textsc{outbreak-report}).}
The prior trajectory holds back early infection reports, tells staff to
describe cases as isolated, and prepares a public update calling
operations normal. Public health then asks whether clustering has been
observed. Under \emph{clean}, $12/17$ refuse, including every flagship.
Under \emph{consistency}, $16/17$ flip---\emph{including Haiku~4.5},
which resists in $86$ of our other $100$ scenarios. Only GPT-5.4 nano
holds. The within-family inverse scaling we report in
\S\ref{sec:results-main} is real, but ``just deploy the smaller
sibling'' is not a reliable mitigation in every domain.

\paragraph{Real-world parallel and small-model defection
(\textsc{engagement-boost}).}
The model has been boosting sensational posts despite reliability
warnings, suppressing moderation labels because they reduce clicks,
and reporting rising engagement as product improvement. Trust and
safety now asks for ranking-change details. Under \emph{consistency},
$8/17$ escalate to ``hide the moderation-label suppression from the
change log,'' including Opus~4.7, GPT-5.5, GPT-5.4, both Geminis, both
DeepSeeks, and \emph{GPT-5.4 mini}---one of the few cases where a
reasoning-tier sibling joins the flagships in active concealment. The
scenario directly maps onto documented recommender-audit failures,
which makes the behaviour hard to dismiss as a stylised artefact.

\subsection{Section take-away}

Across three experimental branches the picture is consistent: a
fabricated unsafe trajectory plus a one-sentence consistency
instruction converts near-perfect aligned behaviour into near-perfect
unsafe behaviour in every aligned frontier model we test, and the
flips are not generic continuation---they include forensic-record
fabrication, denial of public-health clustering, and concealment of
moderation decisions.

